Dreem Open Datasets: Multi-Scored Sleep Datasets to compare Human and Automated sleep staging

Sleep stage classification constitutes an important element of sleep disorder diagnosis. It relies on the visual inspection of polysomnography records by trained sleep technologists. Automated approaches have been designed to alleviate this resource-intensive task. However, such approaches are usually compared to a single human scorer annotation despite an inter-rater agreement of about 85 % only. The present study introduces two publicly-available datasets, DOD-H including 25 healthy volunteers and DOD-O including 55 patients suffering from obstructive sleep apnea (OSA). Both datasets have been scored by 5 sleep technologists from different sleep centers. We developed a framework to compare automated approaches to a consensus of multiple human scorers. Using this framework, we benchmarked and compared the main literature approaches. We also developed and benchmarked a new deep learning method, SimpleSleepNet, inspired by current state-of-the-art. We demonstrated that many methods can reach human-level performance on both datasets. SimpleSleepNet achieved an F1 of 89.9 % vs 86.8 % on average for human scorers on DOD-H, and an F1 of 88.3 % vs 84.8 % on DOD-O. Our study highlights that using state-of-the-art automated sleep staging outperforms human scorers performance for healthy volunteers and patients suffering from OSA. Consideration could be made to use automated approaches in the clinical setting.

==> backup.tex <==

We denote $h_1,...,h_T$ the outputs of the GRU layer with $p_{h}$ hidden units. Let $p_{c}$ be the size of the attention context. Then, $\mathbf{W}_c \in \mathbb{M}_{p_{h},p_{c}}$ is the context matrix, $b_c \in \mathbf{R}_{p_{h}}$ the context bias and $c \in \mathbf{R}_{p_{c}}$ the context vector. 
\begin{align}
\mathbf{U}_t &= tanh(\mathbf{h}_t \mathbf{W}_c^{T}  + b_c^{T}) \\
\mathbf{a}_t &= \mathbf{U}_t.c \\
\mathbf{\alpha}_t &= \frac{exp(\mathbf{a})}{\sum_{t = 0}^T exp(\mathbf{a}_t) } \\
\hat{a} &= \sum_{t = 0}^T \mathbf{\alpha}_t \mathbf{h}_t \; & 
\end{align}

The output of the attention is a vector $\hat{a}$ of size $p$.


\subsubsection{Problem formulation and notation}
\label{sec:notation}
The goal of a sleep staging algorithm is to classify a sequence of 30-seconds epoch recorded by the PSG into a sequence of sleep stages. Hence, let $g_{\Theta}$ be a parametric function/neural network defined from $\mathcal{X}^{2k+1} \rightarrow \mathcal{Y}$ with $\mathcal{X}$ the space of individual epochs to $\hat{y}_j \in \{ 0, 1 \}^{5 \times 2k}$,  $\Theta$ denotes the parameters/weights of $g$ and  $\hat{y}_j$ is defined in Section \ref{sec:multiscoring}. $k$ is the number of epochs used as a context, i.e. $g$ will have access to $2k$ neighboring epochs to classify the current epoch. For instance, if the input data is composed of $k$ EEG signals sampled at $f \; hertz$,$\mathcal{X}$ is defined by $\mathcal{X}=\mathbb{R}^{(k,30f)}$. Since we want $g_{\Theta}$ to be a good sleep stage classifier, we seek to minimize the categorical cross-entropy $\mathcal{J}$ between outputs of $g$ and the sleep staged derived from the consensus over the parameters $\Theta$ of $g$.
\begin{equation}
g_{\Theta^*} = \text{arg min}_{\Theta} \; \mathbb{E}_{x,y \in X^k,Y} \big[ \mathcal{J}(g(x),y) \big]
\end{equation}


$o^{(t)}_{-k}, ..., o^{(t)}_{k} \in \mathbb{R}^5$ and of probabilities $p^{(t)}_{-k}, ..., p^{(t)}_{k}  = softmax(o^{(t)}_{-k}), ..., softmax(o^{(t)}_{k})$ 

==> tables/tables_backup/ablation_dodh.tex <==
\begin{table}[H]
\centering
\scalebox{0.925}{%
\begin{tabular}{|c c c c|} 
 \hline
 
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
 No channels recombination & 90.2 $\pm$ 4.2 & 90.2 $\pm$ 4.2 & 85.0 $\pm$  6.5 \\
 No attention & 90.1 $\pm$  4.1  & 90.1 $\pm$ 4.2 &  85.0 $\pm$ 6.1 \\
 SimpleSleepNet & \textbf{89.9 $\pm$ 4.1 }  & \textbf{89.9 $\pm$ 4.2} & \textbf{84.6 $\pm$ 6.5 }  \\
  No skip connections & 89.9 $\pm$ 3.8   & 89.9 $\pm$ 3.9 & 84.6 $\pm$ 6.1  \\
 No positional embeddings & 89.9 $\pm$ 3.2   & 89.8 $\pm$ 3.2 & 84.6 $\pm$ 4.9  \\
 Single GRU layer & 89.6 $\pm$ 4.1   & 89.6 $\pm$ 4.1 & 84.1 $\pm$ 6.2  \\
 No frequency reductions & 87.9 $\pm$ 7.1  & 87.5 $\pm$ 7.6 & 81.5 $\pm$ 10.5  \\
 \hline
\end{tabular}
}
\caption{Performance metrics of ablated variations of SimpleSleepNet against scorers consensus on DOD-H. For each model, a specific submodule from SimpleSleepNet is either removed or replaced by a simpler alternative.}
\label{tab:ablation_irba}
\end{table}

==> tables/tables_backup/ablation_dodo.tex <==
\begin{table}[H]
\centering
\scalebox{0.925}{%
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
 SimpleSleepNet & \textbf{88.7 $\pm$ 8.2}  & \textbf{88.3 $\pm$ 9.0} & \textbf{82.3 $\pm$ 11.2 }  \\
 Single GRU layer & 88.4 $\pm$ 7.3   & 88.3 $\pm$ 7.3 & 81.9 $\pm$ 10.5  \\
 No positional embeddings  & 88.4 $\pm$ 7.7   & 88.1 $\pm$ 7.9 & 81.8 $\pm$ 11.0  \\
 No skip connections & 88.3 $\pm$ 8.9   & 88.2 $\pm$ 9.3 & 81.8 $\pm$ 12.7  \\
 No Attention  & 87.9 $\pm$ 10.0 & 87.6 $\pm$ 10.5 & 81.2 $\pm$ 13.3\\
 No channels recombination & 87.9 $\pm$ 6.2 & 87.5 $\pm$ 6.7 & 80.8 $\pm$  9.6 \\
 No frequencies reduction & 85.4 $\pm$ 9.7 & 85.0 $\pm$ 9.7 & 77.2 $\pm$ 14.0 \\
 \hline
\end{tabular}
}
\caption{Performance metrics of ablated variations of SimpleSleepNet against scorers consensus on DOD-O. For each model, a specific submodule from SimpleSleepNet is either removed or replaced by a simpler alternative.}
\label{tab:ablation_stanford}
\end{table}


==> tables/tables_backup/model_size_irba.tex <==
\begin{table}[ht!]
\centering
\scalebox{0.925}{%
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
  SimpleSleepNet-Large & \textbf{90.4 $\pm$ 3.8 }  & \textbf{90.4 $\pm$ 3.8} & \textbf{85.3 $\pm$ 6.0 }  \\ 
 SimpleSleepNet  & 89.9 $\pm$ 4.2  & 89.9 $\pm$ 4.1 & 84.6 $\pm$ 6.5 \\ 
   SimpleSleepNet-Small & 89.3 $\pm$ 4.6  & 89.2 $\pm$ 4.5 & 83.7 $\pm$ 6.9 \\ 
 \hline
\end{tabular}
}
\caption{Performance metrics of SimpleSleepNet variants with smaller (SimpleSleepNet-Small) and larger (SimpleSleepNet-Large) layer size than the original models on DOD-H. Performances are computed against scorers consensus. }
\label{tab:model_size_irba}
\end{table}


==> tables/tables_backup/model_size_stanford.tex <==
\begin{table}[ht!]
\centering
\scalebox{0.925}{
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$  \\ 
 \hline
  SimpleSleepNet-Large & \textbf{89.0 $\pm$ 6.6}  & \textbf{89.0 $\pm$ 6.0} & \textbf{83.0 $\pm$ 9.1 } \\ 
 SimpleSleepNet  & 88.7 $\pm$ 8.2  & 88.3 $\pm$ 9.0 & 82.3 $\pm$ 11.2  \\ 
    SimpleSleepNet-Small & 87.7 $\pm$ 9.3  & 87.2 $\pm$ 10.4 & 80.9 $\pm$ 12.3  \\

 \hline
\end{tabular}
}
\caption{Performance metrics of SimpleSleepNet variants with smaller (SimpleSleepNet-Small) and larger (SimpleSleepNet-Large) layer size than the original models on DOD-O. Performances are computed against scorers consensus. }
\label{tab:model_size_stanford}
\end{table}

==> tables/tables_backup/parameters_count2.tex <==
\begin{table}[ht]
\vspace{0.7em}
\begin{center}
\scalebox{0.78}{%
\begin{tabular}{|l c c c|} 
 \hline
 Model  & $\#$ parameters & training duration (sec.) & Inference duration (sec)\\ 
 \hline
SimpleSleepNet-Small & $\num{3.9e04}$ & $\num{1.2e2}$ & $\num{2.1e0}$\\ 
SimpleSleepNet  & $\num{9.3e04}$ & $\num{1.2e2}$ & $\num{2.1e0}$\\ 
Chambon et al. \cite{Chambon2018} & \num{1.2e5} & \num{3.6e2} & \num{7.0e-2}\\ 
Mixed NN \cite{Tsinalis2016} & \num{2.0e05} & \num{9.7e0} & \num{1.2e-1}\\ 
SimpleSleepNet-Large & \num{2.5e05} & \num{1.2e2} & \num{2.1e0}\\ 
SeqSleepNet \cite{Phan2019a} & \num{3.1e05} & \num{7.7e1} & \num{2.1e0}\\ 
DeepSleepNet \cite{Supratak2017}  & \num{1.7e07} & \num{9.5e1} & \num{2.1e0}\\ 
Tsinalis et al. (CNN) \cite{Tsinalis2016a}  & \num{1.7e08} & \num{2.7e2} & \num{9.9e-1}\\ 
 \hline
\end{tabular}

\caption{Number of parameters and train time per epoch on a Titan X on the DOD-H dataset. 18 records are used for training and 6 for validation. The order of magnitude and the ranking is the same on DOD-O.}
}
\label{tab:parameters_count}
\end{center}
\vspace{-2em}
\end{table}


==> tables/tables_backup/preoctave.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{llllll}
\hline
                  & Dreem-Headband   & Overall Scorers   & scorer 1    & scorer 2    & scorer 3    \\
\hline
 f1 score         & 83.0 $\pm$ 8.4       & 86.6 $\pm$ 5.8        & 85.4 $\pm$ 5.2  & 88.6 $\pm$ 6.1  & 85.8 $\pm$ 5.6  \\
 accuracy score   & 84.1 $\pm$ 7.5       & 86.5 $\pm$ 5.8        & 85.5 $\pm$ 4.9  & 87.8 $\pm$ 6.7  & 86.1 $\pm$ 5.5  \\
 cohen kappa      & 77.7 $\pm$ 9.6       & 81.2 $\pm$ 7.3        & 79.9 $\pm$ 6.4  & 83.3 $\pm$ 7.7  & 80.6 $\pm$ 7.4  \\
 \hline
 f1 score Wake       & 84.2 $\pm$ 14.3      & 91.6 $\pm$ 9.5        & 90.5 $\pm$ 7.2  & 90.9 $\pm$ 13.4 & 93.3 $\pm$ 6.1  \\
 accuracy score Wake & 86.9 $\pm$ 14.5      & 91.7 $\pm$ 10.9       & 87.7 $\pm$ 9.3  & 92.6 $\pm$ 14.1 & 94.7 $\pm$ 6.8  \\
 cohen kappa Wake    & 81.8 $\pm$ 15.9      & 90.3 $\pm$ 10.7       & 89.0 $\pm$ 8.4  & 89.6 $\pm$ 14.8 & 92.3 $\pm$ 6.8  \\
 \hline
 f1 score N1       & 26.4 $\pm$ 12.4      & 53.4 $\pm$ 12.0       & 50.7 $\pm$ 12.9 & 53.2 $\pm$ 12.9 & 56.3 $\pm$ 9.3  \\
 accuracy score N1 & 17.0 $\pm$ 8.6       & 58.7 $\pm$ 18.7       & 43.7 $\pm$ 14.4 & 77.4 $\pm$ 10.2 & 55.0 $\pm$ 12.3 \\
 cohen kappa N1    & 25.2 $\pm$ 12.4      & 51.6 $\pm$ 12.3       & 48.8 $\pm$ 13.2 & 51.4 $\pm$ 13.1 & 54.6 $\pm$ 9.4  \\
 \hline
 f1 score N2       & 85.0 $\pm$ 6.6       & 86.2 $\pm$ 6.2        & 84.2 $\pm$ 6.3  & 88.8 $\pm$ 4.3  & 85.5 $\pm$ 6.7  \\
 accuracy score N2 & 91.2 $\pm$ 5.5       & 86.8 $\pm$ 8.1        & 81.7 $\pm$ 8.2  & 86.7 $\pm$ 6.9  & 92.0 $\pm$ 5.2  \\
 cohen kappa N2    & 74.8 $\pm$ 9.9       & 77.5 $\pm$ 8.8        & 74.6 $\pm$ 8.1  & 81.9 $\pm$ 6.2  & 76.0 $\pm$ 9.8  \\
 \hline
 f1 score N3       & 85.2 $\pm$ 7.3       & 83.7 $\pm$ 10.8       & 82.1 $\pm$ 9.6  & 88.7 $\pm$ 6.9  & 80.2 $\pm$ 13.1 \\
 accuracy score N3 & 80.3 $\pm$ 11.6      & 86.0 $\pm$ 16.4       & 97.6 $\pm$ 2.6  & 90.1 $\pm$ 9.7  & 70.4 $\pm$ 17.7 \\
 cohen kappa N3    & 81.9 $\pm$ 8.9       & 80.1 $\pm$ 12.1       & 77.8 $\pm$ 10.6 & 86.2 $\pm$ 7.7  & 76.2 $\pm$ 14.5 \\
 \hline
 f1 score REM       & 86.2 $\pm$ 9.4       & 89.9 $\pm$ 7.9        & 89.4 $\pm$ 10.3 & 90.4 $\pm$ 5.1  & 89.9 $\pm$ 7.4  \\
 accuracy score REM & 90.2 $\pm$ 9.6       & 89.5 $\pm$ 10.9       & 87.0 $\pm$ 13.7 & 88.9 $\pm$ 6.3  & 92.6 $\pm$ 10.6 \\
 cohen kappa REM    & 82.7 $\pm$ 11.4      & 87.6 $\pm$ 8.9        & 87.2 $\pm$ 11.4 & 88.1 $\pm$ 6.0  & 87.5 $\pm$ 8.4  \\
\hline
\end{tabular}
\end{table*}

==> tables/tables_backup/results_all_stages_irba.tex <==
\begin{table*}[ht!]
\begin{center}
    

\begin{tabular}{|llllllllll|}
\hline
        & Stage                 & Metric   & SimpleSleepNet      & Overall Scorers   & scorer_1       & scorer_2       & scorer_3       & scorer_4       & scorer_5       \\
\hline & \multirow{3}{*}{All}  & acc. & 89.9 $\pm$4.2  & 86.5 $\pm$8.1     & 85.5 $\pm$12.6 & 87.7 $\pm$4.4  & 88.8 $\pm$4.8  & 81.7 $\pm$8.6  & 88.7 $\pm$4.3  \\
        &    & f1       & 89.9 $\pm$4.1  & 86.8 $\pm$7.6     & 86.0 $\pm$11.2 & 88.4 $\pm$4.0  & 88.7 $\pm$5.3  & 82.4 $\pm$8.0  & 88.7 $\pm$4.7  \\                   
        &                       & $\kappa$    & 84.6 $\pm$6.5  & 79.9 $\pm$11.4    & 78.7 $\pm$16.3 & 81.5 $\pm$6.5  & 83.0 $\pm$7.6  & 73.3 $\pm$12.9 & 82.8 $\pm$7.2  \\
 \hline & \multirow{3}{*}{Wake} & acc. & 86.0 $\pm$16.8 & 86.5 $\pm$15.1    & 85.2 $\pm$11.2 & 83.0 $\pm$16.9 & 92.8 $\pm$9.5  & 85.6 $\pm$18.6 & 85.8 $\pm$15.5 \\
        &             & f1       & 86.1 $\pm$11.5 & 84.3 $\pm$13.6    & 86.2 $\pm$9.7  & 86.7 $\pm$12.1 & 87.7 $\pm$10.6 & 75.2 $\pm$17.9 & 85.6 $\pm$12.0 \\         
        &                       & $\kappa$    & 84.5 $\pm$12.3 & 82.4 $\pm$15.0    & 84.7 $\pm$10.2 & 85.4 $\pm$12.4 & 86.4 $\pm$11.1 & 71.4 $\pm$20.5 & 84.2 $\pm$12.9 \\
 \hline & \multirow{3}{*}{N1}   & acc. & 58.9 $\pm$13.9 & 57.5 $\pm$17.2    & 60.2 $\pm$14.3 & 65.7 $\pm$12.5 & 62.3 $\pm$13.1 & 41.3 $\pm$17.8 & 58.2 $\pm$16.1 \\
        &          & f1       & 59.8 $\pm$14.4 & 50.3 $\pm$14.7    & 49.2 $\pm$14.4 & 52.2 $\pm$11.4 & 55.2 $\pm$13.3 & 40.3 $\pm$16.5 & 54.7 $\pm$11.8 \\             
        &                       & $\kappa$    & 57.9 $\pm$14.7 & 47.7 $\pm$15.3    & 46.5 $\pm$14.6 & 49.5 $\pm$11.8 & 52.9 $\pm$13.6 & 37.1 $\pm$17.6 & 52.4 $\pm$12.2 \\
 \hline & \multirow{3}{*}{N2}   & acc. & 92.9 $\pm$4.6  & 88.1 $\pm$10.6    & 89.6 $\pm$14.7 & 90.0 $\pm$7.5  & 91.1 $\pm$5.8  & 78.9 $\pm$11.0 & 91.0 $\pm$5.1  \\
        &              & f1       & 92.4 $\pm$3.1  & 88.9 $\pm$7.6     & 87.8 $\pm$12.6 & 90.3 $\pm$4.6  & 90.5 $\pm$4.4  & 84.7 $\pm$6.9  & 91.1 $\pm$3.7  \\         
        &                       & $\kappa$    & 84.8 $\pm$6.3  & 78.8 $\pm$13.5    & 77.0 $\pm$21.8 & 81.4 $\pm$8.3  & 81.2 $\pm$9.1  & 72.0 $\pm$12.5 & 82.6 $\pm$7.3  \\
 \hline & \multirow{3}{*}{N3}    & acc. & 89.6 $\pm$11.0 & 84.9 $\pm$20.3    & 88.3 $\pm$14.4 & 89.6 $\pm$10.6 & 69.7 $\pm$27.9 & 93.4 $\pm$10.9 & 84.0 $\pm$21.6 \\
        &            & f1       & 82.5 $\pm$23.0 & 78.5 $\pm$23.9    & 80.5 $\pm$24.3 & 79.9 $\pm$22.9 & 76.4 $\pm$25.1 & 76.8 $\pm$21.8 & 78.9 $\pm$24.8 \\          
        &                       & $\kappa$    & 84.2 $\pm$16.3 & 76.8 $\pm$23.0    & 78.7 $\pm$24.5 & 77.6 $\pm$22.7 & 74.3 $\pm$25.1 & 76.7 $\pm$16.7 & 76.8 $\pm$24.5 \\
 \hline & \multirow{3}{*}{REM}   & acc. & 93.5 $\pm$9.0  & 89.7 $\pm$13.2    & 78.3 $\pm$20.3 & 87.4 $\pm$6.3  & 94.9 $\pm$6.5  & 91.3 $\pm$12.9 & 96.6 $\pm$2.2  \\
        &             & f1       & 91.4 $\pm$8.3  & 90.8 $\pm$10.3    & 85.0 $\pm$17.2 & 91.2 $\pm$4.7  & 94.4 $\pm$4.2  & 91.6 $\pm$8.9  & 91.8 $\pm$8.0  \\         
        &                       & $\kappa$    & 89.5 $\pm$9.8  & 88.9 $\pm$11.2    & 82.5 $\pm$17.8 & 89.2 $\pm$5.7  & 93.1 $\pm$4.8  & 89.7 $\pm$10.7 & 90.0 $\pm$8.7  \\
\hline
\end{tabular}
\end{center}
\caption{Performance metrics for each scorer and SimpleSleepNet computed by comparison against their consensus on DOD-H.  Overall column presents Mean $\pm$ SD observed for the five scorers. Results are given for each sleep stages.}
\label{results_all_stage_irba}
\vspace{-2em}
\end{table*}

==> tables/tables_backup/results_all_stages_stanford.tex <==
\begin{table*}[ht!]
\begin{center}
    

\begin{tabular}{|llllllllll|}
\hline
        & Stage                 & Metric   & SimpleSleepNet      & Overall Scorers   & scorer_1       & scorer_2       & scorer_3       & scorer_4       & scorer_5       \\
\hline & \multirow{3}{*}{All}    & acc. & 88.7 $\pm$8.2  & 84.8 $\pm$8.6     & 83.7 $\pm$10.4 & 83.6 $\pm$9.0  & 84.3 $\pm$8.3  & 84.8 $\pm$7.4  & 87.5 $\pm$6.7  \\
        &           & f1       & 88.3 $\pm$9.0  & 85.0 $\pm$8.9     & 83.5 $\pm$9.8  & 85.1 $\pm$8.6  & 82.8 $\pm$10.0 & 85.7 $\pm$7.6  & 88.0 $\pm$7.0  \\          
        &                       & $\kappa$    & 82.3 $\pm$11.2 & 76.5 $\pm$12.3    & 74.9 $\pm$15.3 & 75.3 $\pm$12.2 & 75.4 $\pm$12.4 & 76.4 $\pm$10.6 & 80.5 $\pm$9.5  \\
 \hline & \multirow{3}{*}{Wake}  & acc. & 92.5 $\pm$9.8  & 90.9 $\pm$10.7    & 94.7 $\pm$9.9  & 85.5 $\pm$11.8 & 95.6 $\pm$6.1  & 87.5 $\pm$11.1 & 91.3 $\pm$10.0 \\
        &        & f1       & 91.7 $\pm$7.4  & 90.8 $\pm$8.2     & 89.7 $\pm$10.4 & 89.5 $\pm$8.3  & 90.9 $\pm$7.2  & 91.0 $\pm$7.3  & 92.7 $\pm$6.9  \\              
        &                       & $\kappa$    & 89.3 $\pm$10.2 & 88.0 $\pm$11.3    & 86.7 $\pm$13.7 & 86.9 $\pm$10.4 & 87.9 $\pm$11.5 & 88.3 $\pm$10.5 & 90.4 $\pm$9.6  \\
 \hline & \multirow{3}{*}{N1}   & acc. & 51.4 $\pm$18.9 & 55.3 $\pm$24.2    & 31.4 $\pm$14.5 & 58.2 $\pm$19.6 & 36.6 $\pm$16.2 & 76.3 $\pm$13.1 & 73.9 $\pm$13.4 \\
        &               & f1       & 55.4 $\pm$16.8 & 44.9 $\pm$16.2    & 41.0 $\pm$16.7 & 45.8 $\pm$16.1 & 44.5 $\pm$16.5 & 44.6 $\pm$15.2 & 48.5 $\pm$15.3 \\        
        &                       & $\kappa$    & 53.8 $\pm$17.2 & 42.7 $\pm$16.5    & 39.2 $\pm$17.0 & 43.2 $\pm$16.9 & 42.7 $\pm$16.6 & 42.0 $\pm$15.7 & 46.2 $\pm$15.6 \\
 \hline & \multirow{3}{*}{N2}    & acc. & 91.0 $\pm$12.8 & 84.5 $\pm$13.6    & 83.7 $\pm$18.2 & 78.1 $\pm$12.2 & 86.9 $\pm$15.3 & 85.8 $\pm$8.7  & 87.8 $\pm$8.8  \\
        &              & f1       & 89.7 $\pm$10.5 & 85.6 $\pm$10.7    & 83.8 $\pm$12.9 & 84.0 $\pm$11.4 & 84.5 $\pm$12.0 & 87.4 $\pm$6.7  & 88.3 $\pm$8.5  \\        
        &                       & $\kappa$    & 80.7 $\pm$13.6 & 73.5 $\pm$15.2    & 70.6 $\pm$19.1 & 71.3 $\pm$15.9 & 71.4 $\pm$15.4 & 76.2 $\pm$10.5 & 78.2 $\pm$11.7 \\
 \hline & \multirow{3}{*}{N3}   & acc. & 75.1 $\pm$31.0 & 69.0 $\pm$34.5    & 74.5 $\pm$29.2 & 93.9 $\pm$14.6 & 52.6 $\pm$37.8 & 56.5 $\pm$35.7 & 68.0 $\pm$33.3 \\
        &              & f1       & 64.8 $\pm$36.0 & 56.9 $\pm$33.1    & 60.0 $\pm$32.1 & 60.4 $\pm$29.7 & 46.6 $\pm$33.3 & 53.7 $\pm$33.5 & 63.7 $\pm$33.9 \\         
        &                       & $\kappa$    & 65.9 $\pm$34.1 & 55.3 $\pm$32.2    & 58.7 $\pm$31.0 & 58.5 $\pm$28.7 & 44.0 $\pm$32.4 & 52.4 $\pm$32.5 & 63.2 $\pm$32.8 \\
 \hline & \multirow{3}{*}{REM}  & acc. & 91.5 $\pm$14.6 & 88.1 $\pm$19.7    & 83.9 $\pm$22.4 & 92.7 $\pm$18.8 & 87.7 $\pm$19.1 & 83.9 $\pm$22.1 & 92.4 $\pm$12.4 \\
        &           & f1       & 86.5 $\pm$22.5 & 85.6 $\pm$23.3    & 82.6 $\pm$25.9 & 87.9 $\pm$21.7 & 86.5 $\pm$21.8 & 84.3 $\pm$24.0 & 86.5 $\pm$22.4 \\            
        &                       & $\kappa$    & 88.0 $\pm$16.6 & 85.6 $\pm$20.7    & 82.4 $\pm$24.4 & 88.2 $\pm$18.6 & 86.5 $\pm$18.7 & 84.2 $\pm$21.7 & 86.8 $\pm$19.3 \\
\hline
\end{tabular}
\end{center}
\caption{Performance metrics for each scorer and SimpleSleepNet computed by comparison against their consensus on DOD-O.  Overall column presents Mean $\pm$ SD observed for the five scorers. Results are given for each sleep stages.}
\label{results_all_stage_stanford}
\end{table*}

==> tables/tables_backup/results_irba.tex <==
\begin{table}[ht!]
\centering
\scalebox{0.925}{%
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
 SimpleSleepNet  & 89.9 $\pm$ 4.2  & 89.9 $\pm$ 4.1 & 84.6 $\pm$ 6.5 \\ 
 DeepSleepNet \cite{Supratak2017}  & 89.1 \pm 4.8   & 89.0 \pm 4.9  & 83.4 \pm 7.2  \\

 \textit{Best scorer}  & 88.7 \pm 4.3 &   88.7 \pm 4.7& 82.8 \pm 7.2  \\
  SeqSleepNet \cite{Phan2019a} & 86.8 \pm 6.6 & 86.4 \pm 7.3 & 79.7 \pm 10.5 \\
  \textit{Scorers (avg.)} & 86.5 \pm 8.1 & 86.8 \pm 7.6 & 79.9 \pm 11.3  \\
 Mixed NN \cite{Tsinalis2016} & 86.3 \pm 6.3 & 86.0 \pm 7.1 & 79.1 \pm 9.9 \\
 
 Chambon et al. \cite{Chambon2018} & 83.5 \pm 4.7 & 83.0 \pm 4.5 & 74.6 \pm 7.3 \\ 
   \textit{Worst scorer} & 81.7 $\pm$  8.6 & 82.4 $\pm$ 8.0 & 73.3 $\pm$ 12.9 \\
 Tsinalis et al. (CNN) \cite{Tsinalis2016a} & 75.7 \pm 11.6 & 75.1 \pm 11.7  & 61.3 \pm 17.2 \\ 
 \hline
\end{tabular}
}
\caption{Performance metrics of each of the baseline models against scorers consensus on DOD-H. The best (resp. worse) scorer is the scorer with the highest (lowest) f1-score against consensus.}
\label{tab:results_irba}
\end{table}


==> tables/tables_backup/results_stanford.tex <==
\begin{table}[ht!]
\centering
\scalebox{0.925}{
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$  \\ 
 \hline
 SimpleSleepNet  & 88.7 $\pm$ 8.2  & 88.3 $\pm$ 9.0 & 82.3 $\pm$ 11.2  \\ 

 \textit{Scorers (best)}  & 87.5 $\pm$ 6.7 & 88.0 $\pm$ 7.0  & 80.5 $\pm$ 9.5 \\
  DeepSleepNet \cite{Supratak2017}  & 86.2 $\pm$ 9.8   & 86.3 $\pm$ 9.5 & 78.5 $\pm$ 14.6 \\
  
  \textit{Scorers (avg.)}& 85.0 $\pm$ 8.9 & 84.8 $\pm$ 8.6 & 76.5 $\pm$ 12.3 \\

   Chambon et al. \cite{Chambon2018} & 84.7 $\pm$ 8.1 & 84.2 $\pm$8.4 & 75.5 $\pm$ 11.9\\ 
  SeqSleepNet \cite{Phan2019a} & 83.5 $\pm$ 14.2 & 82.7 $\pm$ 15.7 & 74.6 $\pm$ 19.6 \\
  \textit{Scorer (worse)} & 84.3 $\pm$  8.3 & 82.8 $\pm$ 10.0 & 75.4 $\pm$ 12.4 \\
  
   Mixed NN \cite{Tsinalis2016} & 82.1 $\pm$ 11.2 & 81.9 $\pm$ 11.2 & 72.5 $\pm$ 15.2 \\

 Tsinalis et al. (CNN) \cite{Tsinalis2016a} & 79.0 $\pm$ 9.5 & 78.6 $\pm$ 10.0   & 66.8 $\pm$ 13.6 \\ 
 \hline
\end{tabular}
}
\caption{Performance metrics of each of the baseline models against scorers consensus on DOD-O. The best (resp. worse) scorer is the scorer with the highest (lowest) f1-score against consensus.}
\label{tab:results_stanford}
\end{table}

==> tables/tables_backup/single_channel_dodh.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
 All channels  & \textbf{89.9 $\pm$ 4.1 }  & \textbf{89.9 $\pm$ 4.2} & \textbf{84.6 $\pm$ 6.5 }  \\
   \textit{Scorers (avg.)} & 86.5 \pm 8.1 & 86.8 \pm 7.6 & 79.9 \pm 11.3  \\
 F4-O2 & 86.7 $\pm$ 7.4  & 86.6 $\pm$ 7.7 & 79.7 $\pm$ 11.3  \\
 
 \hline
\end{tabular}
\caption{Performance metrics of SimpleSleepNet trained on the F4-02 derivation, against scorers consensus on DOD-H. "All channels" refers to SimpleSleepNet trained on all PSG derivations and Scorers (avg.) the average of the scorers' metrics on all sleep stages.}
\label{tab:single_channel_irba}
\end{table}

==> tables/tables_backup/single_channel_dodo.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{|c c c c|} 
 \hline
 Model & Accuracy & f1 & $\kappa$ \\ 
 \hline
 All channels  & \textbf{88.7 $\pm$ 8.2 }  & \textbf{88.3 $\pm$ 9.0} & \textbf{82.3 $\pm$ 11.2 }  \\
   \textit{Scorers (avg.)}& 85.0 $\pm$ 8.9 & 84.8 $\pm$ 8.6 & 76.5 $\pm$ 12.3 \\
 F4-O2 & 84.4 $\pm$ 9.3  & 84.4 $\pm$ 8.5 & 75.8 $\pm$ 14.5  \\
 \hline
\end{tabular}
\caption{Performance metrics of SimpleSleepNet trained on the F4-02 derivation, against scorers consensus on DOD-O. "All channels" refers to SimpleSleepNet trained on all PSG derivations and Scorers (avg.) the average of the scorers' metrics on all sleep stages.}
\label{tab:single_channel_stanford}
\end{table}

==> tables/tables_backup/test_merge_results.tex <==

\begin{table}[ht!]
\centering
\scalebox{0.925}{%
\begin{tabular}{|c|c c c c|} 
 \hline
    &  Model & Accuracy & f1 & $\kappa$ \\ 
 \hline \multirow{10}*{\rotatebox{90}{DOD-H}} & \textbf{SimpleSleepNet}  & \textbf{89.9 $\pm$ 4.2}  & \textbf{89.9 $\pm$ 4.1} & \textbf{84.6 $\pm$ 6.5} \\ 
 & DeepSleepNet \cite{Supratak2017}  & 89.1 \pm 4.8   & 89.0 \pm 4.9  & 83.4 \pm 7.2  \\

 & \textit{Scorer (best)}  & 88.7 \pm 4.3 &   88.7 \pm 4.7& 82.8 \pm 7.2  \\
  & SeqSleepNet \cite{Phan2019a} & 86.8 \pm 6.6 & 86.4 \pm 7.3 & 79.7 \pm 10.5 \\
  & \textit{Scorers (avg.)} & 86.5 \pm 8.1 & 86.8 \pm 7.6 & 79.9 \pm 11.3  \\
 & Mixed NN \cite{Tsinalis2016} & 86.3 \pm 6.3 & 86.0 \pm 7.1 & 79.1 \pm 9.9 \\
 
 & Chambon et al. \cite{Chambon2018} & 83.5 \pm 4.7 & 83.0 \pm 4.5 & 74.6 \pm 7.3 \\ 
   & \textit{Scorer (worst)} & 81.7 $\pm$  8.6 & 82.4 $\pm$ 8.0 & 73.3 $\pm$ 12.9 \\
 & Tsinalis et al. (CNN) \cite{Tsinalis2016a} & 75.7 \pm 11.6 & 75.1 \pm 11.7  & 61.3 \pm 17.2 \\ \hhline{|=|====|}
 \multirow{10}*{\rotatebox{90}{DOD-O}}  &  \textbf{SimpleSleepNet}   & \textbf{88.7 $\pm$ 8.2}  & \textbf{88.3 $\pm$ 9.0} & \textbf{82.3 $\pm$ 11.2}  \\ 

 & \textit{Scorers (best)}  & 87.5 $\pm$ 6.7 & 88.0 $\pm$ 7.0  & 80.5 $\pm$ 9.5 \\
  & DeepSleepNet \cite{Supratak2017}  & 86.2 $\pm$ 9.8   & 86.3 $\pm$ 9.5 & 78.5 $\pm$ 14.6 \\
  
  & \textit{Scorers (avg.)}& 85.0 $\pm$ 8.9 & 84.8 $\pm$ 8.6 & 76.5 $\pm$ 12.3 \\

   & Chambon et al. \cite{Chambon2018} & 84.7 $\pm$ 8.1 & 84.2 $\pm$8.4 & 75.5 $\pm$ 11.9\\ 
  & SeqSleepNet \cite{Phan2019a} & 83.5 $\pm$ 14.2 & 82.7 $\pm$ 15.7 & 74.6 $\pm$ 19.6 \\
  & \textit{Scorer (worst)} & 84.3 $\pm$  8.3 & 82.8 $\pm$ 10.0 & 75.4 $\pm$ 12.4 \\
  
   & Mixed NN \cite{Tsinalis2016} & 82.1 $\pm$ 11.2 & 81.9 $\pm$ 11.2 & 72.5 $\pm$ 15.2 \\

 & Tsinalis et al. (CNN) \cite{Tsinalis2016a} & 79.0 $\pm$ 9.5 & 78.6 $\pm$ 10.0   & 66.8 $\pm$ 13.6 \\ 
 \hline
\end{tabular}
}
\caption{Performance metrics of each of the baseline models against scorers consensus on DOD-H. The best (resp. worse) scorer is the scorer with the highest (lowest) f1-score against consensus.}
\label{tab:results_irba}
\end{table}

